MMD Guidance: Training-Free Distribution Adaptation for Diffusion Models via Maximum Mean Discrepancy Guidance

Pre-trained diffusion models have emerged as powerful generative priors for both unconditional and conditional sample generation, yet their outputs often deviate from the characteristics of user-specific target data. Such mismatches are especially problematic in domain adaptation tasks, where only a few reference examples are available and retraining the diffusion model is infeasible. Existing inference-time guidance methods can adjust sampling trajectories, but they typically optimize surrogate objectives such as classifier likelihoods rather than directly aligning with the target distribution. We propose \emph{MMD Guidance}, a training-free mechanism that augments the reverse diffusion process with gradients of the \textit{Maximum Mean Discrepancy (MMD)} between generated samples and a reference dataset. MMD provides reliable distributional estimates from limited data, exhibits low variance in practice, and is efficiently differentiable, which makes it particularly well-suited for the guidance task. Our framework naturally extends to prompt-aware adaptation in conditional generation models via product kernels. Also, it can be applied with computational efficiency in latent diffusion models (LDMs), since guidance is applied in the latent space of the LDM. Experiments on synthetic and real-world benchmarks demonstrate that MMD Guidance can achieve distributional alignment while preserving sample fidelity. The project code is available at github.com/matinamehdizadeh/MMD-Guidance.

==> sections/5-theory.tex <==
\subsection{MMD Guidance as McKean--Vlasov Langevin Dynamics}

We consider the mean-field (population) form of MMD-guided Langevin dynamics
\begin{equation}
\label{eq:mv-langevin}
dX_t = \left( \nabla \log p(X_t) - \lambda\, G_k(X_t;\mu_t,\nu) \right)dt + \sqrt{2}\,dW_t,
\end{equation}
where $\mu_t$ is the law of $X_t$, $\nu$ is a fixed target law, and
\begin{equation}
\label{eq:Gk-def}
G_k(x;\mu,\nu) := 2\left( \mathbb{E}_{X'\sim \mu}[\nabla_1 k(x,X')] - \mathbb{E}_{Y\sim \nu}[\nabla_1 k(x,Y)] \right).
\end{equation}
Equation~\eqref{eq:mv-langevin} is a McKean--Vlasov SDE since the drift depends on the current law $\mu_t$ via $G_k$.

\subsection{Polynomial Kernel Expansion and Moment Tensors}

Throughout this subsection, let the kernel be the (inhomogeneous) degree-$r$ polynomial kernel
\begin{equation}
\label{eq:poly-kernel}
k_r(x,y) = (c + \langle x,y\rangle)^r \qquad (c\geq 0,\; r\in\mathbb{N}).
\end{equation}
For a distribution $\rho$ on $\mathbb{R}^d$, we write its order-$m$ moment tensor as
\[
M_m(\rho) := \mathbb{E}_{Z\sim \rho}[Z^{\otimes m}] \in (\mathbb{R}^d)^{\otimes m}.
\]
We use the notation
\[
\mathcal{C}_{s}(M_{s+1}(\rho); x) := M_{s+1}(\rho) \times_1 x \times_2 x \cdots \times_s x \in \mathbb{R}^d
\]
for the contraction of the $(s+1)$-tensor $M_{s+1}(\rho)$ with $x^{\otimes s}$ along $s$ indices, yielding a vector in $\mathbb{R}^d$.

\begin{lemma}[Polynomial kernel gradient as a moment polynomial]
\label{lem:poly-gradient}
Let $k_r$ be as in \eqref{eq:poly-kernel}. Then for any probability measures $\mu,\nu$ with finite moments up to order $r$,
\begin{equation}
\label{eq:Gk-moment-expansion}
G_{k_r}(x;\mu,\nu) = 2r \sum_{s=0}^{r-1} \binom{r-1}{s} c^{r-1-s} \left( \mathcal{C}_{s}(M_{s+1}(\mu); x) - \mathcal{C}_{s}(M_{s+1}(\nu); x) \right)
\end{equation}
for all $x\in\mathbb{R}^d$. In particular, $G_{k_r}(x;\mu,\nu)$ is a polynomial vector field in $x$ of degree at most $r-1$, with coefficients linear in the moment differences $M_{m}(\mu)-M_{m}(\nu)$ for $m=1,\ldots,r$.
\end{lemma}

\begin{proof}
For $k_r(x,y)=(c+\langle x,y\rangle)^r$, we have
\[
\nabla_1 k_r(x,y) = r(c+\langle x,y\rangle)^{r-1}y.
\]
By the binomial expansion,
\begin{align*}
(c+\langle x,y\rangle)^{r-1} &= \sum_{s=0}^{r-1} \binom{r-1}{s} c^{r-1-s} \langle x,y\rangle^s\\
&= \sum_{s=0}^{r-1} \binom{r-1}{s} c^{r-1-s} \langle x^{\otimes s}, y^{\otimes s}\rangle.
\end{align*}
Hence,
\begin{align*}
\mathbb{E}_{Y\sim \rho}[\nabla_1 k_r(x,Y)] &= r \sum_{s=0}^{r-1} \binom{r-1}{s} c^{r-1-s} \mathbb{E}[\langle x^{\otimes s}, Y^{\otimes s}\rangle Y]\\
&= r \sum_{s=0}^{r-1} \binom{r-1}{s} c^{r-1-s} \mathcal{C}_{s}(M_{s+1}(\rho); x).
\end{align*}
Subtracting the $\nu$-expectation from the $\mu$-expectation and multiplying by 2 yields \eqref{eq:Gk-moment-expansion}.
\end{proof}

\subsection{Exponential Families with Polynomial Sufficient Statistics}

Consider the regular exponential family
\begin{equation}
\label{eq:exp-family}
p_\theta(x) = h(x)\exp\left(\sum_{|\alpha|\leq r} \theta_\alpha x^\alpha - A(\theta)\right),
\end{equation}
where $\alpha$ is a multi-index, $x^\alpha=\prod_{j=1}^d x_j^{\alpha_j}$, and $T_\alpha(x)=x^\alpha$ for $|\alpha|\leq r$ are the sufficient statistics. We assume $\nabla \log h(x)$ is a polynomial vector field of degree at most $r-1$.

The score field is then
\begin{equation}
\label{eq:score-expfam}
\nabla \log p_\theta(x) = \nabla \log h(x) + \sum_{|\alpha|\leq r} \theta_\alpha \nabla x^\alpha,
\end{equation}
which is a polynomial vector field of degree at most $r-1$. The collection $\{\nabla x^\alpha: 1\leq |\alpha|\leq r\}$ spans all polynomial vector fields of degree at most $r-1$, with the explicit identity
\begin{equation}
\label{eq:monomial-basis-identity}
\frac{\partial}{\partial x_\ell} x^{\gamma+e_\ell} = (\gamma_\ell+1) x^\gamma, \qquad 0\leq |\gamma|\leq r-1, \;\ell\in[d].
\end{equation}

\subsection{Exact Score Adaptation and Moment Matching}

\begin{theorem}[Exact score adaptation within the same exponential family]
\label{thm:score-adaptation}
Fix $r\in\mathbb{N}$ and the degree-$r$ polynomial kernel $k_r$ in \eqref{eq:poly-kernel}. Let $\nu$ be any target law with finite moments up to order $r$. Let $p_\theta$ be the exponential family \eqref{eq:exp-family} with sufficient statistics $\{x^\alpha:|\alpha|\leq r\}$ and assume $\nabla \log h$ has degree at most $r-1$.

For any probability measure $\mu$ with finite moments up to order $r$, expand $G_{k_r}(x;\mu,\nu)$ uniquely in the monomial vector basis $\{x^\gamma e_\ell: 0\leq |\gamma|\leq r-1, \ell\in[d]\}$:
\begin{equation}
\label{eq:G-expansion}
G_{k_r}(x;\mu,\nu) = \sum_{\ell=1}^d \sum_{0\leq |\gamma|\leq r-1} g_{\ell,\gamma}(\mu,\nu) x^\gamma e_\ell,
\end{equation}
where the coefficients $g_{\ell,\gamma}$ depend linearly on the moment differences $\{M_m(\mu)-M_m(\nu)\}_{m=1}^r$ by Lemma~\ref{lem:poly-gradient}.

Then there exists a unique parameter vector $\widetilde\theta(\mu)\in\mathbb{R}^{\{|\alpha|\leq r\}}$ of the form
\begin{equation}
\label{eq:theta-tilde}
\widetilde\theta_{\gamma+e_\ell}(\mu) = \theta_{\gamma+e_\ell} - \lambda \frac{g_{\ell,\gamma}(\mu,\nu)}{\gamma_\ell+1}, \quad \text{for all } \ell\in[d], 0\leq |\gamma|\leq r-1,
\end{equation}
(and $\widetilde\theta_0(\mu)=\theta_0$ if $0\in\{|\alpha|\leq r\}$) such that the pointwise identity
\begin{equation}
\label{eq:score-equality}
\nabla \log p_{\widetilde\theta(\mu)}(x) = \nabla \log p_\theta(x) - \lambda G_{k_r}(x;\mu,\nu)
\end{equation}
holds for all $x\in\mathbb{R}^d$.

Consequently, if at time $t$ the law $\mu_t$ lies in the family $\{p_\theta\}$, the MMD-guided drift in \eqref{eq:mv-langevin} is exactly the score of another member of the same exponential family.
\end{theorem}

\begin{proof}
By Lemma~\ref{lem:poly-gradient}, $G_{k_r}(\cdot;\mu,\nu)$ is a polynomial vector field of degree at most $r-1$, with unique expansion \eqref{eq:G-expansion}. By \eqref{eq:monomial-basis-identity},
\[
\nabla x^{\gamma+e_\ell} = (\gamma_\ell+1) x^\gamma e_\ell,
\]
so the set $\{\nabla x^{\gamma+e_\ell}\}$ forms a basis for polynomial vector fields of degree at most $r-1$. For each coefficient pair $(\ell,\gamma)$, we match terms by choosing $\widetilde\theta$ as in \eqref{eq:theta-tilde}. Substituting into the score representation \eqref{eq:score-expfam} gives identity \eqref{eq:score-equality}. Uniqueness follows from linear independence of the basis. If $M_m(\mu)=M_m(\nu)$ for all $m\leq r$, then all $g_{\ell,\gamma}(\mu,\nu)=0$ and $\widetilde\theta(\mu)=\theta$, so $G_{k_r}(\cdot;\mu,\nu)\equiv 0$.
\end{proof}

\subsection{Degree-2 (Quadratic) Kernel and Gaussian Closure}

We spell out the $r=2$ case explicitly. Let $k_2(x,y)=(c+\langle x,y\rangle)^2$ with $c\geq 0$. Then
\[
\nabla_1 k_2(x,y) = 2(c+\langle x,y\rangle)y, \quad
\mathbb{E}_{Y\sim \rho}[\nabla_1 k_2(x,Y)] = 2\left(c\mathbb{E}[Y] + \mathbb{E}[YY^\top]x\right).
\]
Hence,
\begin{equation}
\label{eq:G2}
G_{k_2}(x;\mu,\nu) = 4\left(\left(\mathbb{E}_\mu[YY^\top]-\mathbb{E}_\nu[YY^\top]\right)x + c\left(\mathbb{E}_\mu[Y]-\mathbb{E}_\nu[Y]\right)\right),
\end{equation}
where $\mathbb{E}_\rho[Y]$ and $\mathbb{E}_\rho[YY^\top]$ denote the first moment and second moment matrix of distribution $\rho$.

If $p_\theta=\mathcal{N}(\mu_p,\Sigma_p)$, its score is affine: $\nabla\log p_\theta(x)= -\Sigma_p^{-1}(x-\mu_p)$. Using \eqref{eq:score-equality} with \eqref{eq:G2}, the adapted score remains affine and corresponds to another Gaussian $\mathcal{N}(\mu_{\text{new}},\Sigma_{\text{new}})$ with
\begin{align}
\label{eq:gauss-update}
\Sigma_{\text{new}}^{-1} &= \Sigma_p^{-1} + 4\lambda\left(\mathbb{E}_\mu[YY^\top]-\mathbb{E}_\nu[YY^\top]\right),\\
\Sigma_{\text{new}}^{-1}\mu_{\text{new}} &= \Sigma_p^{-1}\mu_p + 4\lambda c\left(\mathbb{E}_\nu[Y]-\mathbb{E}_\mu[Y]\right). \nonumber
\end{align}
Writing $\mathbb{E}_\rho[YY^\top]=\Sigma_\rho+\mu_\rho\mu_\rho^\top$, equation \eqref{eq:gauss-update} shows that quadratic-kernel guidance shifts the precision by the second-moment mismatch and shifts the mean weighted by the first-moment mismatch.

\iffalse
\subsection{General Moment-Matching Statement}

\begin{theorem}[Moment matching up to order $r$]
\label{thm:moment-matching}
Let $k_r$ be the degree-$r$ polynomial kernel \eqref{eq:poly-kernel} and $p_\theta$ be the exponential family \eqref{eq:exp-family}. Suppose the law $\mu_\star=p_{\theta_\star}$ is a stationary point of the MMD-guided McKean--Vlasov dynamics \eqref{eq:mv-langevin} within the family, i.e., it satisfies
\[
\nabla \log p_{\theta_\star}(x) \equiv \nabla \log p_{\theta}(x) - \lambda G_{k_r}(x;\mu_\star,\nu).
\]
Then necessarily
\[
M_m(\mu_\star) = M_m(\nu), \qquad m=1,\ldots,r.
\]
Equivalently, $\text{MMD}_{k_r}(\mu_\star,\nu)=0$.
\end{theorem}

\begin{proof}
By Theorem~\ref{thm:score-adaptation}, the score identity holds with coefficients $g_{\ell,\gamma}(\mu_\star,\nu)$ from \eqref{eq:G-expansion}. Comparing coefficients in the monomial basis shows $g_{\ell,\gamma}(\mu_\star,\nu)=0$ for all $(\ell,\gamma)$. 

By Lemma~\ref{lem:poly-gradient}, each $g_{\ell,\gamma}$ is a linear combination of moment differences $\{M_m(\mu_\star)-M_m(\nu)\}_{m\leq r}$. The triangular structure of \eqref{eq:Gk-moment-expansion}—where the term with index $s$ depends only on $M_{s+1}$—allows us to solve sequentially: first $M_1(\mu_\star)=M_1(\nu)$ from $s=0$ terms, then $M_2(\mu_\star)=M_2(\nu)$ from $s=1$ terms, and so on up to $M_r(\mu_\star)=M_r(\nu)$.

The equivalence with $\text{MMD}_{k_r}(\mu_\star,\nu)=0$ follows because the feature map of $k_r$ consists of all monomials up to degree $r$, so the kernel mean embedding encodes precisely the moments up to order $r$.
\end{proof}

\subsection{Finite-Sample Implementation}

In practice, we replace population moments by empirical moments. For generated samples $\{z_t^{(i)}\}_{i=1}^B$ and reference samples $\{z_j^{(r)}\}_{j=1}^{N_r}$, define empirical moment tensors:
\[
\widehat{M}_m(\widehat{P}_t) = \frac{1}{B}\sum_{i=1}^B (z_t^{(i)})^{\otimes m}, \quad
\widehat{M}_m(\widehat{Q}) = \frac{1}{N_r}\sum_{j=1}^{N_r} (z_j^{(r)})^{\otimes m}.
\]

Lemma~\ref{lem:poly-gradient} holds with $M_m$ replaced by $\widehat{M}_m$, and the parameter update \eqref{eq:theta-tilde} uses these empirical statistics. Standard concentration inequalities (e.g., matrix Bernstein) give deviation bounds:
\[
\|\widehat{M}_m(\widehat{P}_t) - M_m(\mu_t)\|_{\text{op}} = O_p\left(\sqrt{\frac{m! \cdot d^m}{B}}\right),
\]
and similarly for reference samples with rate $O_p(1/\sqrt{N_r})$.

\fi
